Workload-Aware Systems and Interfaces for Cognitive Augmentation

In today's society, our cognition is constantly influenced by information intake, attention switching, and task interruptions. This increases the difficulty of a given task, adding to the existing workload and leading to compromised cognitive performances. The human body expresses the use of cognitive resources through physiological responses when confronted with a plethora of cognitive workload. This temporarily mobilizes additional resources to deal with the workload at the cost of accelerated mental exhaustion. We predict that recent developments in physiological sensing will increasingly create user interfaces that are aware of the user's cognitive capacities, hence able to intervene when high or low states of cognitive workload are detected. Subsequently, we investigate suitable feedback modalities in a user-centric design process which are desirable for cognitive assistance. We then investigate different physiological sensing modalities to enable suitable real-time assessments of cognitive workload. We provide evidence that the human brain and eye gaze are sensitive to fluctuations in cognitive resting states. We show that electroencephalography and eye tracking are reliable modalities to assess mental workload during user interface operation. In the end, we present applications that regulate cognitive workload in home and work setting, investigate how cognitive workload can be visualized to the user, and show how cognitive workload measurements can be used to predict the efficiency of information intake through reading interfaces. Finally, we present our vision of future workload-aware interfaces. Previous interfaces were limited in their ability to utilize cognitive workload for user interaction. Together with the collected data sets, this thesis paves the way for methodical and technical tools that integrate workload-awareness as a factor for context-aware systems.

==> chapter/00_misc/acros.tex <==
\DeclareAcronym{SUS}{short = SUS, long =  System Usability Scale}
\DeclareAcronym{6DoF}{short = 6DoF , long = six degree of freedom}
\DeclareAcronym{HCI}{short = HCI , long = Human-Computer Interaction}
\DeclareAcronym{TCT}{short = TCT , long = task completion time}
\DeclareAcronym{TLX}{short = NASA-TLX , long = NASA Task Load Index}
\DeclareAcronym{IV}{short = IV , long = independent variable}
\DeclareAcronym{DV}{short = DV , long = dependent variable}
\DeclareAcronym{LHRD}{short = LHRD, long = large high-resolution display}
\DeclareAcronym{UI}{short = UI, long = user interface}
\DeclareAcronym{GP}{short = GP, long = Gaussian Processes}
\DeclareAcronym{NN}{short = NN, long =  neural network}
\DeclareAcronym{NNR}{short = NNR, long =  neural network regression}
\DeclareAcronym{KNN}{short = KNN, long =  K-Nearest-Neighbor}
\DeclareAcronym{ReLU}{short = ReLU, long =  rectified linear unit}

==> chapter/00_misc/layout-definitions.tex <==
\definecolor{primaryColor}{HTML}{A2C2DE}
\definecolor{secondaryColor}{HTML}{E1EAF4}
\definecolor{tertiaryColor}{HTML}{cbd6e5}
%\definecolor{tertiaryColor}{HTML}{F3F7FB}
\definecolor{MyGray}{rgb}{0.86,0.87,0.88}

\definecolor{ReferenceGray}{rgb}{0.91,0.91,0.91}

\makeatletter\newenvironment{graybox}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{.8\columnwidth}}{
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\makeatletter\newenvironment{grayboxwide}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{\textwidth}}{
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\makeatletter\newenvironment{definitionbox}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{.88\textwidth}	\vspace{3mm}}{
	\vspace{3mm}
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\makeatletter\newenvironment{referencebox}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{.98\textwidth}	\vspace{3mm}}{
	\vspace{3mm}
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\newcommand{\publicationsbegin}{ 
   \begin{list}{\raise .5ex\hbox{\scriptsize$\bullet$}}
    { \setlength{\itemsep}{5pt}      \setlength{\parsep}{3pt} 
      \setlength{\topsep}{6pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.7em} } }

\newcommand{\publicationsend}{
    \end{list}  } 

\newcommand{\etal}{\mbox{et al.\,}\xspace}

==> chapter/__latexindent_temp.tex <==
% !TEX root = ../thesis.tex

%\input{chapter/06_case03/01_case03_intro}

\chapter{Smooth Pursuits}
\label{ch:smooth_pursuit}

\epigraph{\textit{The eyes are the mirror of the soul and reflect everything that seems to be hidden; and like a mirror, they also reflect the person looking into them.}}{Paulo Coelho}

The previous chapter investigated the feasibility of \ac{EEG} signals as a measure for cognitive workload. The analysis of cortical activity has proved useful to detect changes in cognitive demand in real-time. Thereby, \ac{EEG} provides the capability to derive the mental demand directly from the brain. However, \ac{EEG} relies on a correct setup of the headset that has to be kept steady to avoid noise in the signal. Other factors, such as head movements and eye movements, may influence the signal as well. Therefore, alternative modalities have been juxtaposed to overcome the limitations that \ac{EEG} measures pose.

As such, eye tracking has emerged as both inferences for cognitive states as well as an interaction modality. Eye gaze-based interactive systems hold a lot of promise for cognition-aware interaction~\cite{bulling2014cognition}. The human eye represents the central organ which enables visual processing. Complemented by previous research, eye gaze as an input for interactive systems has been extensively explored~\cite{duchowski2002breadth}. One specific eye movements, namely smooth pursuit eye movements, have been utilized as an alternative eye movement input modality for interactive systems~\cite{hutchinson1989human, vidal2013pursuits}. In contrast to \ac{EEG}, smooth pursuit has the advantage to be a contactless measure. Eye movements can be recorded using a remote eye tracker, neglecting the need for hardware that has to be attached to the user. Furthermore, smooth pursuit eye movements cannot be pretended since they require locking onto a moving target~\cite{velloso2016ambigaze}. This robustness against false positives is another benefit of using smooth pursuit eye movement as an interaction technique.

\begin{figure}
    \includegraphics[width=\columnwidth]{figures/all_trajectories.png}
        \vspace{-1em}
    \caption[Example of smooth pursuit recordings for different workload levels]{Smooth pursuit recordings under different levels of cognitive workload for three trajectories. The blue line shows the displayed trajectory, while the orange line visualizes the gaze path. (A), (B), and (C) show the gaze path during low cognitive workload phases, while (D), (E), and (F) shows the gaze path during states of high workload.}
    \vspace{-1em}
    \label{fig:teaser_intro}
\end{figure}

Research has shown that the behavior of the eye is strongly affected by psychological~\cite{purves2001types, schenck1987rapid} and psychophysiological states of the human body~\cite{sparks2002brainstem, zihl1983selective}. One such state is cognitive workload, which has a remarkable impact on eye movements~\cite{barnes2008cognitive, JUST1976441, stuyven2000effect}. Figure~\ref{fig:teaser_intro} shows how cognitive workload affects smooth pursuit eye movements. Driving in a stressful context or performing multitasking during cognitively demanding tasks under time pressure are just two examples. Previous measures for cognitive workload facilitate questionnaires, such as the NASA-TLX~\cite{doi:10.1177/154193120605000909, HART1988139} or the Driver Activity Load Index (DALI)~\cite{pauzie2008method}, which are often used in \ac{HCI} to evaluate interfaces. Yet these questionnaires are prone to the interpretation of the questions by the user and only allow for an assessment at the end of the task, hence providing rather coarse-grained insights. At the same time, eye-tracking data can be used to assess cognitive workload~\cite{Dingler:2016:CSM:2968219.2968565}. In particular, previous work showed that under controlled conditions, pupil dilation provides an estimate of cognitive load~\cite{peysakhovich2016study, pfleging2016model}. However, pupil dilation is highly sensitive to light conditions, which change in outdoor environments, and hence cannot easily be applied in many ubiquitous computing settings. 

%Other touchless methods that infer cognitive workload via physiological sensing involve heart rate~\cite{KRANJEC2014102} or facial skin temperature measures~\cite{Abdelrahman:2017:CHE:3139486.3130898, stemberger2010thermal}. However, these modalities depend on several other factors, such as constant temperatures or highly controlled environments.

In this chapter, we propose an approach that exploits smooth pursuit eye movements to assess cognitive workload. We hypothesize that working memory, a component of cognitive workload, measurably affects smooth pursuit eye movements~\cite{BADDELEY197447}. Henceforth, we define smooth pursuit describes eye movements that occur as the eyes closely follow a moving object. These movements are evaluated in several studies used for user interface element selection~\cite{esteves2015orbits, velloso2016ambigaze} or intuitive eye tracker calibration~\cite{khamis2016textpursuits, vidal2013pursuits}. By conducting a user study, we found that smooth pursuit can be used for a contactless assessment of cognitive workload with an accuracy of up to $99.5\%$. Thereby, the need for body-worn sensors is obviated. This chapter reports on a user study that investigates the impact of cognitive workload on smooth pursuit eye movements. Based on the insights from the user study we build a classifier to approximate the level of cognitive workload using gaze differences during smooth pursuit eye movements. We discuss how these findings can be used during the evaluations that require the assessment of cognitive workload as well as for the design of cognition-aware interactive systems. This chapter investigates smooth pursuit eye movements as part of the following research question:

\begin{itemize}%[leftmargin=1em]
    \renewcommand{\labelitemi}{$\rightarrow$}
   \item \textbf{RQ4}: Do eye gaze metrics enable the classification of cognitive workload states?
\end{itemize}

\begin{center}
    \begin{GrayBox}
        \centering
        \parbox{0.98\textwidth}{
            \emph{This section is based on the following publication:}
            \vspace{3mm}
            \publicationsbegin    
            \item \bibentry{Kosch:2018:YET:3173574.3174010}
            \publicationsend
        }
    \end{GrayBox}
\end{center}

\section{Related Work}
We present related work concerning existing research on using smooth pursuit eye movements for interaction and the influence of cognitive workload on eye movements.

\subsection{Interacting with Smooth Pursuit}
Using eye gaze as input for ubiquitous interactive systems has been extensively explored. Duchowski~\cite{duchowski2007eye,duchowski2002breadth} performed a literature survey about current eye-tracking applications and technologies. Focusing on usability, related research shows how eye tracking technologies evolved until they became usable in human-computer interaction research~\cite{jacob2003eye, poole2006eye}.
Recent research has addressed the use of eye gaze for selection tasks~\cite{ohno1998features,sibert2000evaluation}, which can be used by physiologically impaired individuals to perform input on computers~\cite{hutchinson1989human}. Text input via eye input has been researched using dwell time~\cite{bee2008writing, majaranta2002twenty}, off-screen targets~\cite{isokoski2000text}, or eye movements along the y-axis on a display~\cite{tuisku2008now}. The usage of such methods was also evaluated in real-world scenarios~\cite{de2007evaluation,zhang2013sideways}. Furthermore, eye movements and eye gestures can be used to interact with devices.

Recently, smooth pursuit eye movement~\cite{hutchinson1989human,vidal2013pursuits} has been used as an alternative gaze-based input modality to interactive systems. This interaction technique overcomes the need for precise calibration and training of the user before interaction and further supports ubiquitous interaction. Several researchers have investigated how smooth pursuits can be used intuitively. People cannot pretend to perform smooth pursuit movements since they require locking onto a moving target~\cite{velloso2016ambigaze}. This reduces the likeliness of detecting false positives during an interaction. 

Another approach to leverage smooth pursuit as an input modality has been researched by Esteves et al.~\cite{esteves2015orbits}. They used a mobile eye tracker to enable hands-free interaction with a smartwatch by showing moving dots on the smartwatch display. Results show robustness against false positives regarding input, no need for calibrating an eye tracker, and efficient hands-free interaction. Using smooth pursuit to interact with physical real-world devices also showed promising results. Velloso et al. \cite{velloso2016ambigaze} developed and evaluated an object-driven system, which can be operated by only performing smooth pursuit. As soon as a user approaches an object such as a fan or windmill, it begins to present moving targets that trigger actions as soon as selected by smooth pursuit.

Researchers have also used smooth pursuit to calibrate eye trackers. Pfeuffer et al.~\cite{pfeuffer2013pursuit} investigated this approach by using animations on a display to implicitly calibrate an eye tracker. Their results state that a 5-point calibration achieved a higher detection rate and required less calibration time. They concluded that smooth pursuits calibration provides better usability and flexibility for eye tracker calibration on small displays.   

Vidal et al.~\cite{vidal2013pursuits} proposed different applications for smooth pursuit eye interaction, such as selection tasks or password authentication. The implemented applications showed a fast selection and completion time for different tasks. % A user study with different applications shows a fast selection and completion time for different tasks. 
Since smooth pursuit can be performed with almost every kind of animated trajectory, more recently Khamis et al.~\cite{khamis2016textpursuits} investigated which trajectories are most suitable for smooth pursuit interaction and calibration when showing text-based content on a display. While showing a question in the top left corner of a screen, they also showed several answers to the question on the same screen displayed in different trajectories. Schenk et al.~\cite{Schenk:2017:GEG:3025453.3025455} used smooth pursuit as an element selection mechanism in desktop settings to avoid the Midas touch problem~\cite{Jacob:1990:YLY:97243.97246}. Similarly, Lohr and Komogortsev~\cite{Lohr:2017:CSP:3027063.3053233} compared smooth pursuit-based input against dwell-based input approaches. A significant faster selection of elements was achieved when using smooth pursuit at the cost of likely unwanted selections.


\subsection{Impact of Cognitive Workload on Eye-based Properties}
Previous research has shown that the behavior of the eye is strongly affected by the psychological~\cite{purves2001types, schenck1987rapid} and psycho-physiological~\cite{sparks2002brainstem,zihl1983selective} state of the human body. One such state is cognitive workload, which has a shown impact on eye movements~\cite{barnes2008cognitive,stuyven2000effect}.

Researchers found a relation between pupillary responses and cognitive demand~\cite{ahern1979pupillary, hess1964pupil}. During a task comprising different task complexities, the pupil diameter of participants was measured as an indicator for cognitive workload.
Results show increasing pupil dilation with increasing task difficulty. Pfleging et al.~\cite{pfleging2016model} created a model to estimate cognitive workload under different lighting conditions based on pupil dilation. The feasibility of measuring pupil dilation using a remote eye tracker has been investigated by Klingner et al.~\cite{klingner2008measuring}. Their findings show a lower accuracy compared to mobile eye trackers due to noise and head movements. Kruger et al. \cite{kruger2013measuring} investigated eye behavior when perceiving a stimulus with and without subtitles using electroencephalography and pupillary measurements. In an experiment with two groups, lower cognitive workload was measured within the group perceiving subtitles than in the group lacking subtitles.

Liang and Lee~\cite{liang2008driver} compared the efficiency of different machine learning algorithms to estimate distractions during driving tasks based on saccadic eye movements. Higher frequencies of saccadic eye movements have been used as an assessment for cognitive workload. Best results were achieved using a \ac{SVM} for machine learning. However, their findings address saccadic eye movements only and do not examine the effects of smooth pursuit eye movements under cognitive workload. 

Benedetto et al. \cite{benedetto2011driver} investigated the correlation between blink duration and visual and cognitive workload of a driver operating a car in a simulated environment. Participants had to perform a Lane Change Test~\cite{mattes2009surrogate} while doing an in-vehicle information system task~\cite{Victor2005167} at the same time. Their findings show a lower blink duration compared to their baseline task than in the cognitively demanding task. Ahlstrom and Friedman-Berg \cite{ahlstrom2006using} also found a significant correlation between shorter blink durations and cognitive workload. 

Stuyven et al. \cite{stuyven2000effect} investigated the impact of cognitive workload on saccadic eye movements. Their findings show an increased occurrence of saccadic eye movements when inducing cognitive workload. Tsai et al.~\cite{tsai2007task} investigated how eyes behave under cognitive workload while performing a paced auditory serial addition task~\cite{gronwall1977paced}, however, their work did not investigate the impact on smooth pursuit eye movements. Recently, Zagermann et al.~\cite{10.1145/2993901.2993908} developed a model and showed concepts to derive cognitive workload from eye behavior, such as saccades, fixations, pupil dilation, and eye blinks. Cognitive workload influences microsaccadic eye movements \cite{siegenthaler2014task}. They found that microsaccades occur more frequently with higher perceived workload during a non-visual task.

The voluntary involvement of smooth pursuit eye movements has been researched by Barnes~\cite{barnes2008cognitive}. He showed that cognitive processes in smooth pursuit eye movements are even involved without voluntary participation. Important factors for following moving stimuli were attention and awareness, which trigger the process of smooth pursuit on a neuro-scientific level. Therefore, smooth pursuit eye movements are voluntary up to a certain degree. In contrast, Collewijn and Tamminga~\cite{collewijn1984human} investigated contexts in which smooth pursuit movements are voluntary. They used different targets and backgrounds to investigate smooth pursuit performances of humans. Contreras et al.~\cite{contreras2011effect} researched the eye-target synchronization performance of people with traumatic brain injury. People suffering from traumatic brain injuries show a worse performance when performing smooth pursuit in terms of deviation points apart from a shown moving object on a display.

Previous work has investigated how smooth pursuit can be leveraged for calibration and interaction. However, to our knowledge, no prior work has proposed to use work to propose using smooth pursuit eye movements as a measurement to derive cognitive workload. This opens new opportunities for researchers and practitioners alike. In particular, using smooth pursuits as a real-time measurement for cognitive workload is valuable in the context of evaluating interactive systems as well as for developing cognitively adaptive systems.

\label{sec:evaluation}
\section{Study}

To understand the impact of cognitive workload on smooth pursuit eye movements, we designed a lab user study where we induced cognitive workload while participants performed smooth pursuit eye movements.

\subsection{Independent Variables}
In our experiment on investigating the impact of cognitive workload on eye movements, we explore the influence of three independent variables when interacting with smooth pursuit systems: (1) trajectory type~\cite{khamis2016textpursuits}, (2) speed of the stimulus~\cite{khamis2015field}, and (3) task difficulty. In the following, we describe these three independent variables in detail.

\begin{figure}
    \includegraphics[width=\columnwidth]{figures/trajectories.png}%\hspace{12pt}
    \caption[Smooth pursuit trajectories used in the study]{Three different trajectories chosen for evaluation: (A) Rectangular trajectory, (B) Circular trajectory, (C) Sinusoidal trajectory. The size of the moving object in the experiment was 10\,pixels.}
    \label{fig:trajectories}
    \vspace{-1em}
\end{figure}

\subsubsection{Trajectories}
Since smooth pursuit eye movements can be triggered by showing a stimulus moving along a particular trajectory, we implemented a rectangular, a circular, and a sine wave animation to produce this effect. We have chosen these trajectories based on previous research~\cite{khamis2015field,khamis2016textpursuits,vidal2013pursuits}. Furthermore, the chosen trajectories may have a physiological effect paired with the current task difficulty, since the human eye has six muscles responsible for horizontal and vertical movements as well as eye rotations~\cite{leigh2015neurology}. Rectangular trajectories demand muscles on the left and right side of the eye for horizontal movements, while vertical movements demand the upper and lower eye muscles. Circular and sinusoidal eye movements demand four muscles around the eye. Rectangular trajectories require horizontal or vertical movements only, while circular and sinusoidal include diagonal movements as well. In the context of leveraging smooth pursuit as interaction modality, the presented trajectories are used to distinguish between different user inputs. The chosen trajectories are depicted in Figure \ref{fig:trajectories}.

\begin{figure*}
    \centering
        \includegraphics[width=\columnwidth]{figures/study_procedure2.pdf}
        \caption[Study procedure]{Study procedure. First, consent approval and demographic data were collected. Afterward, a baseline task was conducted followed by a set of six trials, where each trial differs in trajectory speed and task complexity. This procedure is repeated for every remaining trajectory type.}
        \label{fig:study_procedure}
\end{figure*}

\subsubsection{Speed of Stimulus}
We compare two different speeds at which stimuli are moving based on previous research~\cite{khamis2015field}: $450\,\frac{px}{s}$ (slow\footnote{This corresponds to $17.14^\circ$ per second at a viewing distance of approximately 50 centimeters}) and $650\,\frac{px}{s}$ (fast\footnote{This corresponds to $24.76^\circ$ per second at a viewing distance of approximately 50 centimeters}). Displaying slower or faster animations while experiencing cognitive workload can lead to different performances since eye muscles have to deal with different strains per speed and trajectory~\cite{leigh2015neurology}. Furthermore, trajectory speeds can be used to differentiate user input, since eye movements adapt to different speeds.

\subsubsection{Task Difficulty}
To induce cognitive workload, we use an auditory delayed digit recall \textit{N}-back task from Mehler et al.~\cite{mehler2011agelab} with an English-spoken number set. The \textit{N}-back task is a commonly used task to artificially elicit working memory resources~\cite{BADDELEY197447}, a component of cognitive workload which strains temporal memory capacities and affects secondary task performances negatively~\cite{berka2007eeg,brouwer2012estimating,turner1989working}.

Throughout the study, we use the \textit{N}-back task to manipulate cognitive workload by demanding working memory with different difficulty levels~\cite{kane2007working}. For each trial, participants hear randomized numbers consisting of ten digits between 0 and 9. Hereby, \textit{N} corresponds to the \textit{N}-last digit. After hearing the number, participants have to say out loud the digit they heard \textit{N} digits ago. In our experiment, we use a \textit{1}-back, \textit{2}-back, and \textit{3}-back tasks to induce cognitive workload. By increasing \textit{N}, more digits have to be remembered, hence increasing task difficulty. To collect baseline measures, participants were asked to follow a trajectory without performing an \textit{N}-back task. Similar as in the study presented in Chapter~\ref{ch:workloadbyeeg}, Table \ref{tab:nback2} shows an example of the \textit{N}-back task.

\renewcommand{\arraystretch}{1.2}
\begin{table}[h!]
 \begin{center}
 \begin{tabular}{l|c|c|c|c|c|c|c}
   \toprule
   \textbf{Heard number} & 5 & 8 & 3 & 4 & 3 & 9 & 1\\
   \hline
   \textbf{Number to say (\textit{1}-back task)} & & 5 & 8 & 3 & 4 & 3 & 9 \\
   \hline
   \textbf{Number to say (\textit{2}-back task)} & & & 5 & 8 & 3 & 4 & 3 \\
   \hline
   \textbf{Number to say (\textit{3}-back task)} & & & & 5 & 8 & 3 & 4 \\
   \bottomrule
 \end{tabular}
   \caption{Example of the auditory delayed digit recall \textit{N}-back task. Participants have to remember the \textit{N}-th number back of a spoken number sequence and say the number out loud.}
 \label{tab:nback2}
 \end{center}
 \vspace{-1em}
\end{table}

\subsection{Apparatus}
The study was conducted in a quiet lab with no windows, where lighting conditions were fixed. The setting was spatially divided into an experimenter area and a participant area. A separator divided both areas. While the experimenter controlled the experiment using a laptop, the participant saw an animated trajectory on a 22\,inch screen with a resolution of $1680\,\times\,1050$\,pixels and a refresh rate of 60\,\ac{Hz}. Eye gaze data was collected using a RED250 from SensoMotoric Instruments with a sample rate of 250\,\ac{Hz}. No filter was applied to the captured gaze data, thus raw gaze data was recorded only. We used a Holosonic Audio Spotlight 24i directed speaker to provide the auditory delayed digit recall \textit{N}-back task. 
%The experimental setup is depicted in Figure \ref{fig:experimentsetup}.

\subsection{Method and Measures}
We used a repeated-measures design with three independent variables as described in the previous section; namely trajectory (rectangular, circular, sine wave), speed (slow, fast), and cognitive workload (no task, \textit{1}-back task, \textit{2}-back task, \textit{3}-back task). Each experiment consisted of three sessions, where animated trajectories were changed for each session. The animated trajectory consisted of a white dot with a diameter of 10\,pixels. The background was set to gray (RGB: [128,128,128]) to avoid eye exhaustion caused by screen brightness.

Before starting a new session, the eye tracker was calibrated to retrieve gaze points for later analysis of gaze deviations between baseline and smooth pursuit eye movements. Each session began with a 30\,second baseline trial, where the animated trajectory used for the session was shown to participants without inducing cognitive workload. This allowed us to estimate eye movement differences from the displayed trajectory when no cognitive workload was present. We chose a slow speed ($450\,\frac{px}{s}$) to make participants familiar with the displayed trajectory.

Cognitive workload was induced by providing a task difficulty using the auditory \textit{N}-back task described in the prior section while showing the animated trajectory at a certain speed. Task difficulty and speed were counterbalanced during a session according to the Latin square, while each session showed the same trajectory. The order of sessions was counterbalanced participant-wise according to the Latin square. This resulted in seven trials per session, including the baseline task. Running all three sessions, the experiment comprised 21 trials per participant. Overall, the duration of each trial was 25 to 30 seconds, dependent on the length of the spoken number for tasks including task difficulty. After completing a trial, participants were asked to fill out a NASA-TLX questionnaire to assess subjectively perceived cognitive workload. Participants took a 30-second long break afterward. Figure~\ref{fig:study_procedure} shows an illustration of the study procedure.


\subsection{Participants}
We recruited 20 participants (9 female, 11 male), aged between 22 and 34 years (M = $27.5$, SD = $3.13$). Before the experiment, each participant signed a consent form and provided their demographic data. All participants were computer science, students or researchers. All participants had a normal or corrected-to-normal vision. Participants were recruited through university mailing lists. They received sweets and five Euro as compensation. The duration of the study was approximately 30 minutes. 
We explained the purpose of the study and tasks to the participants and informed them they could exit the study at any point. Participants signed informed consent forms and were seated in a comfortable chair, approximately 50 centimeters in front of the display before the experimental setup. Due to technical issues, two participants were excluded from the analysis, as their gaze data was not recorded properly.


\section{Results}
We analyze our data to compare the impact of trajectory type, speed, and task difficulty on smooth pursuit eye movements. We report on quantitative results by comparing measured eye gaze data with the showed trajectory. This is complemented by a subjective analysis through NASA-TLX questionnaires.

\begin{table}
\begin{center}
    \begin{tabular}{lc}
        \toprule
        \textbf{Paired Wilcoxon Signed-Rank Test} & \textbf{Significance}\\
        \midrule
        \begin{tabular}{l|l} Circle Baseline & Circle \textit{1}-back fast \end{tabular} & $p = .002$\\ 

        \begin{tabular}{l|l} Circle Baseline & Circle \textit{2}-back fast \end{tabular} & $p = .002$\\

        \begin{tabular}{l|l} Circle Baseline & Circle \textit{3}-back fast \end{tabular} & $p = .003$\\

        \begin{tabular}{l|l} Circle Baseline & Circle \textit{2}-back slow \end{tabular} & $p = .004$\\ 

        \begin{tabular}{l|l} Circle Baseline & Circle \textit{3}-back slow \end{tabular} & $p = .005$\\

        \begin{tabular}{l|l} Sine Baseline \hspace{1.5mm} & Sine \textit{1}-back fast \end{tabular} & $p < .001$\\ 

        \begin{tabular}{l|l} Sine Baseline \hspace{1.5mm} & Sine \textit{2}-back fast \end{tabular} & $p < .001$\\

        \begin{tabular}{l|l} Sine Baseline \hspace{1.5mm} & Sine \textit{3}-back fast \end{tabular} & $p < .001$\\

        \begin{tabular}{l|l} Sine Baseline \hspace{1.5mm} & Sine \textit{1}-back slow \end{tabular} & $p = .003$\\

        \begin{tabular}{l|l} Sine Baseline \hspace{1.5mm} & Sine \textit{2}-back slow \end{tabular} & $p = .002$\\

        \begin{tabular}{l|l} Sine Baseline \hspace{1.5mm} & Sine \textit{3}-back slow \end{tabular} & $p = .002$\\
        \bottomrule
    \end{tabular}
    \caption[Summary of significant results between the workload levels]{Summary of significant results. Comparisons between other conditions did not result in significant differences.    
}
    \label{tab:significantresults}
    \end{center}
    \vspace{-1em}
\end{table}

\subsection{Smooth Pursuit Differences and Cognitive Workload}
To evaluate the effect of different task difficulties on smooth pursuit performances, we based our analysis on pixel differences between coordinates of the displayed trajectory and measured eye gaze position at the screen. More formally, we calculated the difference between two coordinates $p$ and $q$ using the Euclidean distance with the formula
\begin{equation} \label{eq:euclidean_distance}
         D = \sqrt{\left(p_{t,x} - q_{t,x}\right)^{2} + \left(p_{t,y} -
   q_{t,y}\right)^{2}}
\end{equation}

where $p$ and $q$ depict a two-dimensional vector comprising the baseline coordinates and measured gaze coordinates from participants. We introduce the variable $t$ describing the temporal dependency between eye gaze and displayed stimulus as the used 250 Hz eye tracker might introduce a temporal offset of four milliseconds, which is below the perceptual threshold for interaction.
Differences were normalized with respect to the maximum gaze deviation %apart
from the shown trajectory. To enable a descriptive analysis, normalized coordinates were averaged for all participants and conditions. Lowest mean eye gaze deviations (M$_{pd}$) were measured for all slow trajectories, where no cognitive workload was induced (Rectangle:~M$_{pd} = 9.14$, SD $= 6.75$, Circle:~M$_{pd} = 9.51$, SD $= 8.03$, Sine:~M$_{pd} = 4.37$, SD $= 1.60$).
Fast rectangular trajectories using a \textit{3}-back task (M$_{pd} = 13.25$, $SD = 11.06$), fast circular trajectories using a \textit{2}-back task (M$_{pd} = 14.54$, SD $= 7.14$) and fast sinusoidal trajectories using a \textit{3}-back task (M$_{pd} = 9.85$, SD $= 3.53$) led to highest mean eye gaze deviations.

Applying a Shapiro-Wilk test on the mean data set showed a non-normal distribution for all conditions (all $p < .05$). A Friedman test showed no significant differences between various levels of cognitive workload and gaze deviations of smooth pursuit eye movements for slow rectangles ($\chi^2(3) = 3.000$, $p = .392$). However, a Friedman test found significant differences within various levels of cognitive workload for fast rectangles ($\chi^2(3) = 11.867$, $p = .008$), slow circles ($\chi^2(3) = 18.867$, $p < .001$), fast circles ($\chi^2(3) = 29.400$, $p < .001$), slow sine waves ($\chi^2(3) = 14.667$, $p = .002$) and fast sine waves ($\chi^2(3) = 30.667$, $p < .001$). We conducted a Wilcoxon signed-rank post hoc test to find significant differences between pairs of task difficulties including baseline trials and normalized gaze deviations after applying a Bonferroni correction (significance level set to $p < .0083$). A summary of significant results can be depicted from Table~\ref{tab:significantresults}. Further, the Cohen's d effect size values of the significant statistical comparisons ranged between $d = 0.66$ and $d = 0.88$.


To visualize averaged relative differences when performing smooth pursuit eye movements, all averaged relative eye movement differences per participant and condition were plotted. This resulted in one data point per participant and per trial, or 21 data points per participant. The averaged plot is depicted in Figure~\ref{fig:errorparticipant}, where the y-axis depicts the gaze deviations from the shown trajectory in percent. The bottom x-axis is annotated with task difficulties and the top x-axis describes trajectory velocities. The trajectory type is color-coded.
% \begin{figure}
%  \includegraphics[width=\columnwidth]{figures/chapter_eye_tracking/averaged_error_per_participant3.pdf}
%  \vspace{-1em}
%  \caption{Scatter plot of the mean gaze deviation per participant and condition. Each dot represents the mean gaze deviations between the recorded and showed the trajectory of a participant. The baseline measurements show a constant behavior and do not scatter apart from the displayed trajectory. Compared to the baseline tasks, circular and sinusoidal trajectories scatter along the y-axis with increasing task difficulty.
%  }
%    \vspace{-1em}
%  \label{fig:errorparticipant}
% \end{figure}


\begin{figure}
    \centering
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/averaged_error_per_participant3.pdf}
        \label{fig:errorparticipant}}
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/tlx_error_participant3.pdf}
        \label{fig:nasatlx}}
    \caption[Averaged eye gaze deviations and raw NASA-TLX scores]{\textbf{(a):} Scatter plot of the mean gaze deviation per participant and condition. Each dot represents the mean gaze deviations between the recorded and showed the trajectory of a participant. The baseline measurements show a constant behavior and do not scatter apart from the displayed trajectory. Compared to the baseline tasks, circular and sinusoidal trajectories scatter along the y-axis with increasing task difficulty. \textbf{(b):} Mean NASA-TLX score for different trajectories, task difficulties, and speeds. Increasing task difficulties led to higher NASA-TLX scores. The error bars depict the standard error.}
    \label{fig:errors_tlx}
\end{figure}

Gaze deviations obtained from baseline trials do not scatter in contrast to gaze deviations measured from trials with task difficulty for circular and sinusoidal trajectories. Furthermore, gaze deviations increase between slow and fast trajectories when raising the task difficulty. However, results show important constraints when assessing cognitive workload from smooth pursuit eye movements. Rectangular trajectories show less eye gaze deviations when increasing task difficulty compared to baseline trials. Thus, evaluating the presence of cognitive workload using rectangular smooth pursuit eye movements is less accurate compared to circular and sinusoidal trajectories. Depending on the setting of a smooth pursuit-driven user interface, rectangular trajectories should be favored when accurate input is required even when the user is impacted by cognitive workload. Circular and sinusoidal trajectories show higher gaze deviations under cognitive workload. Circular and sinusoidal trajectories show clear differences between trials with and without cognitive workload. Such trajectories may be used to determine the existence of cognitive workload.

\subsection{Subjective Analysis of Cognitive Workload}
The lowest NASA-TLX scores per trajectory were subjectively perceived by participants when showing fast rectangles during a \textit{1}-back task (M $= 6.27$, SD $= 4.03$), slow circles during a \textit{1}-back task (M $= 7.13$, SD $= 3.87$), and slow sine waves during a \textit{1}-back task (M $= 5.78$, SD $= 3.41$). Per trajectory, the highest NASA-TLX scores were measured when displaying fast rectangles during a \textit{3}-back task (M $= 12.29$, SD $= 3.97$), fast circles during a \textit{3}-back task (M $= 13.28$, SD $= 3.68$), and fast sine waves during a \textit{3}-back task (M $= 12.63$, SD $= 3.42$). A repeated measures ANOVA showed statistically significant differences between different levels of cognitive workload and NASA-TLX score ($F(2, 321) = 68.503$, $p < .001$). However, no statistically significant differences were found for different speeds ($F(1, 322) = 2.035$, $p = .211$) and displayed trajectories ($F(2, 321) = 21.461$, $p = .722$) compared to NASA-TLX scores. Figure~\ref{fig:nasatlx} illustrates the averaged values from the obtained NASA-TLX scores.

The quantitative analysis shows significant outcomes regarding gaze deviations with different stimuli speeds and \textit{N}-back complexities. To address the impact of different variables on the individual's subjective perception, we conducted a statistical analysis to investigate single NASA-TLX items in correlation to the stimulus speed and \textit{N}-back difficulty. We compare the single NASA-TLX items grouped by the two different speeds. Our results show a significant difference for the \textit{physical demand} ($p = .006$, M$_{slow} = 5.11$, M$_{fast} = 5.69$), \textit{temporal demand} ($p = .003$, M$_{slow} = 7.29$, M$_{fast} = 8.27$), and \textit{effort} ($p = .001$, M$_{slow} = 9.53$, M$_{fast} = 10.29$) scales. However, no significant difference was found in the mental load scale ($p > 0.05$).

To show that different \textit{N}-back difficulties were responsible for higher perceived cognitive workload, we conducted a Wilcoxon signed-rank test to compare the mental NASA-TLX items between the different task complexities. We found significant differences between all three \textit{N}-back difficulties (all $p < .001$) for the \textit{mental demand} scales (M$_{N=1} = 5.84$, M$_{N=2} = 10.56$, M$_{N=3} = 13.84$). Further, we investigate whether the relationship between NASA-TLX scores and gaze deviations was linear using a Pearson correlation. No correlation was found ($.11 < r < .15$, $\forall\,N \in \{1, 2, 3\}$). Thus, it appears that the relationship between the variables is more complex \textit{i.e.} non-linear. This shows the need to understand how smooth pursuit affects subjectively perceived workload.


% \begin{figure}
%  \includegraphics[width=\columnwidth]{figures/chapter_eye_tracking/tlx_error_participant3.pdf}
%    \vspace{-1em}
%  \caption{Mean NASA-TLX score for different trajectories, task difficulties, and speeds. The error bars depict the standard error. Increasing task difficulties led to higher NASA-TLX scores.}
%    \vspace{-1em}
%  \label{fig:nasatlx}
% \end{figure}

\section{Predicting Cognitive Workload}
Results from the study showed significantly increased eye movements during cognitive workload for circular and sinusoidal trajectories. The perception of cognitive workload by the individual is supported by subjective ratings of participants using NASA-TLX questionnaires. We train a classifier that predicts cognitive workload from smooth pursuit eye movements. We investigate the performance of person-dependent and person-independent classification for the different experimental conditions.

\begin{table*}
\begin{center}
    \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
     & \multicolumn{4}{c}{\textbf{Binary Pers.-Indep.}} & \multicolumn{4}{c}{\textbf{Multilabel Pers.-Indep.}} & \multicolumn{2}{c}{\textbf{Multilabel Pers.-Dep.}}\\
    \textbf{Stimulus} & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy & F1 \\
    \midrule
    Rectangle Slow & $75.0\%$ & $37.5\%$ & $50.0\%$ & $42.9\%$ & $40.3\%$ & $26.9\%$ & $40.0\%$ & $30.5\%$ & $48.6\%$ & $52.4\%$\\
    Rectangle Fast & $76.4\%$ & $40.1\%$ & $52.8\%$ & $46.0\%$ & $54.2\%$ & $44.0\%$ & $54.1\%$ & $47.2\%$ & $69.4\%$ & $74.2\%$\\
    Circle Slow & $95.8\%$ & $89.6\%$ & $91.7\%$ & $90.5\%$ & $40.3\%$ & $26.9\%$ & $40.2\%$ & $30.9\%$ & $69.5\%$ & $60.0\%$\\
    Circle Fast & $97.2\%$ & $93.0\%$ & $94.4\%$ & $93.7\%$ & $55.6\%$ & $45.8\%$ & $55.6\%$ & $48.5\%$ & $85.0\%$ & $74.4\%$\\
    Sine Slow & $80.1\%$ & $55.6\%$ & $64.8\%$ & $59.8\%$ & $43.1\%$ & $30.6\%$ & $43.0\%$ & $34.5\%$ & $79.3\%$ & $76.3\%$\\
    Sine Fast & $99.5\%$ & $98.9\%$ & $99.2\%$ & $99.0\%$ & $59.7\%$ & $51.9\%$ & $59.7\%$ & $54.4\%$ & $88.1\%$ & $84.5\%$\\
    \bottomrule
\end{tabular}}\vspace{-1mm}
\caption[Classification performance scores of the eye movement deviation]{Accuracy, precision, recall, and F1 scores of the binary and multi-label person-independent (pers.-indep.) as well as person-dependent (pers.-dep.) classifications. Fast circular and sinusoidal trajectories yield higher classification performances than slower linear trajectories.}
\vspace{-2mm}\label{tab:class_scores}
\end{center}
\end{table*}

\subsection{Attributes, Instances, and Classes}
Data preprocessing was necessary before training a predictive model. We removed the first two seconds per trial to avoid distortions in the signal caused by participants initially searching for the stimulus. We used the collected gaze data and normalized it concerning the coordinates of the shown trajectory. We then calculate the Euclidean distance (see Equation~\ref{eq:euclidean_distance}) between each coordinate of the normalized displayed trajectory and the normalized gaze points recorded from participants. These gaze deviations are defined as the only attribute for the instances we used for classifier training and evaluation later. We smoothed the data using an averaging running window (length 250\,samples) and a hop size of one sample.

The instances used for classifier training and evaluation consisting of a one-dimensional vector, where the normalized gaze deviations represent the only attribute. We define two sets of classes with different class labels. The first class has two labels consisting of \textit{low workload}, referring to trials where no \textit{N}-back task was used, or \textit{high workload}, thus referring to trials including any \textit{N}-back task. We investigate binary classification performances using this class. In contrast, the second class contains the four labels \textit{0-back}, \textit{1-back}, \textit{2-back}, and \textit{3-back}, each referring to the measurements of trials using the corresponding \textit{N}-back task. Overall, we constructed 378 instances, each containing 6000 gaze values, which were used for training and evaluation.

\subsection{Classifier Performance}

An SVM with a linear kernel was used to investigate the prediction performance~\cite{liang2008driver, tsochantaridis2004support, witten2016data}. The previously described instances were used for training and assigned to their appropriate class labels. Within our classifier learning process, we aimed to evaluate the classification efficiency for binary classification, such as detecting low cognitive workload and high cognitive workload. Furthermore, we investigated the classifier performance for determining different levels of cognitive workload concerning the \textit{N}-back task difficulty. We used scikit-learn\footnote{\url{www.scikit-learn.org} - last access \urldate} to train different prediction models.

\subsubsection{Person-Independent Binary Classification}
We performed a person-independent leave-one-person-out classification using two labels; one assigned to low cognitive workload referring to baseline trials and one assigned to high cognitive workload referring to trials comprising a \textit{1}-back, \textit{2}-back, or \textit{3}-back task. A leave-one-person-out classification uses all except one participant for training, while the final participant is used for validating the trained model. The leave-one-person-out classification was carried out for each trajectory and speed separately, where the instances contain the normalized gaze deviations from the shown trajectory per participant and difficulty. The leave-one-person-out classification procedure was repeated for every participant\footnote{Overall 18 runs to use every participant for validation} and the results were averaged. Table~\ref{tab:class_scores} shows the accuracies, precisions, recalls, and F1 scores of the binary classification per trajectory and speed. The classification results favor fast trajectories in combination with changing directions, such as circular or sinusoidal stimuli.

\subsubsection{Person-Independent Multilabel Classification}
To investigate the performance of classifying different levels of cognitive workload, the same leave-one-out validation procedure was conducted for four labels, with each label assigned to instances with their respective task difficulty. Again, the validation was conducted for every participant after using the other participants for training. The results are shown in Table~\ref{tab:class_scores}.

The overall classification efficiency is lower compared to the binary classification accuracy. Different reasons can be responsible for this. First, we are aware that multiple labels may lead to a lower efficiency when the difference between values within the \textit{N}-back conditions is low. Second, we combine multiple participants who may differ in their smooth pursuit behavior individually. The generalized data could, therefore, be biased by individual gaze behavior, which leads to a distorted result. Therefore, we investigate person-dependent training for cognitive workload classification purposes.

\subsubsection{Person-Dependent Multilabel Classification}
We analyzed instances within each person to investigate if higher accuracies could be achieved due to person-dependent properties. Instead of a leave-one-person-out classification, we conducted a leave-one-repetition-out classification for each participant, speed, and trajectory. However, the number of folds had to be set differently, since the animations iterated a different number of times depending on the trajectory and speed\footnote{Each trajectory started and ended at the same position}. Therefore, we adjusted the number of folds of the leave-one-repetition-out classification per trajectory and speed.

The number of folds was set to $k=2$ for slow rectangles, $k=3$ for fast rectangles, $k=5$ for slow circles, $k=7$ for fast circles, $k=2$ for slow sine waves, $k=3$ for fast sine waves. The data per trajectory and speed and participant was randomly partitioned into $k$ folds, where $k-1$ folds were used for training while the last fold was used for evaluation. This procedure was conducted $k$ times per participant and trajectory with the different \textit{N}-back difficulties assigned to the training set. The results were first averaged per participant and then over all participants. Table~\ref{tab:class_scores} shows the results of the cross-validation. Person-dependent classification of multiple cognitive workload levels shows a higher accuracy for fast smooth pursuit movements. Especially fast circular and fast sinusoidal trajectories show better performances compared to rectangular trajectories.

\section{Discussion}
Results from our study show how cognitive workload leads to increased gaze differences of smooth pursuit eye movements during the presence of cognitive workload. We found that faster circular and sinusoidal trajectories led to higher gaze deviations, while rectangular trajectories did not show this effect. We believe, that circular and sinusoidal trajectories required more effort from users since they had to focus more on their task completion due to constantly changing directions. This may be a reason for improved classification results for this kind of trajectories. In contrast, rectangular trajectories can be deployed within smooth pursuit-based interfaces whenever reliable input, independent from the perceived cognitive workload, is required. Depending on the use case, a cognition-aware system designer can decide if reliable input through rectangular trajectories or mental workload estimation by circular and sinusoidal trajectories is desired.

The speed of the trajectories had a quantitative measurable effect on the overall smooth pursuit performances. However, as the statistical investigations of single NASA-TLX scales showed, \textit{mental demand} was not affected compared to \textit{physical} and \textit{temporal demand} as well as \textit{effort} by different speeds. Faster speeds cause therefore a different type of physical workload than cognitive workload which significantly impacts smooth pursuit eye movements. Different trajectory speeds are thus not necessarily responsible for inducing cognitive workload. By comparing different \textit{N}-back difficulties about the NASA-TLX scales, we found a significant difference between all difficulties. This supports, that subjectively perceived cognitive workload was altered by different \textit{N}-back complexities and that both variables manipulate measurable smooth pursuit performances.

The classification results yield higher accuracies for distinguishing between low and high workload levels than for detailed levels of cognitive workload. Furthermore, binary classification can be achieved without the need for person-dependent calibration, while separating different levels of cognitive workload requires a person-dependent calibration regarding cognitive workload.

In a real deployment scenario, binary classification can be used to provide additional help for users when high cognitive workload is classified. This refers to very simple scenarios, where only the estimation of low and high workload is desired. Such places could be public places when, for example, interacting with public displays. In contrast to short interactions in the public, a classifier can be trained for multilevel classifications in private spaces where long-term interaction is conceivable.

Calibrating a classification model with multiple workload levels in the public can result in a cumbersome procedure due to external factors impacting the individual cognitive capacities, such as distracting pedestrians walking by. Our results indicate binary workload classification in the public using a pre-trained classification model, while a classification model with multiple workload levels can be used in private spaces where calibration can be done without any disruptions.

To employ sensing of cognitive workload, smooth pursuit must be elicited. In contrast to smooth pursuit-based user interfaces, other environments require explicit or implicit integration of moving elements. For example, as short waiting times occur as a result of a database query or as a new task is loaded during a user study, feedback on the system status could be presented in a way that fosters smooth pursuit movements. For example, this can be elicited by an animated progress bar. In this way, traditional methods such as the NASA-TLX or DALI questionnaires can be complemented.

Finally, a suitable workload level must be found. Looking back at the classification results of the multi-label model, we achieved reasonable accuracies for person-dependent classification. A cognition-aware system must be able to find the right difficulty for each user, as permanent support by a system may lead to boredom or no support leads to frustration for the user. Keeping the task difficulty at its highest or lowest level might not be favored. However, for deploying binary classification in public use cases minor support might be helpful compared to private settings, where user expectations on cognition-aware computing systems are higher.
\subsection{Limitations}

Our study is prone to certain limitations. We collected gaze data under controlled lab conditions and hence, do not know how our results generalize to other situations, where participants may be distracted for example, by the presence of other people. Still, despite the controlled conditions, participants' gaze behavior may have been influenced by physiological wellbeing, such as lack of sleep. Our calculation of gaze difference is based on 30\,seconds of recording. However, there may be situations in which assessing workload with finer granularity is desirable. Additionally, blink frequency and blink duration were not evaluated during our studies. Another limiting factor was the study execution in a calm lab. Natural distractions in real-world environments could alter our results. Furthermore, we have not investigated the effect of different eye tracking frame rates in our study. Consequently, before assessing cognitive workload through smooth pursuit, eye trackers must be tested for their suitability.

\section{Use Cases for Workload-Aware Systems}
In the following, we present several different use cases to be supported within smooth pursuit scenarios.

\subsection{Support in Safety-Critical Environments}
Smooth pursuit can be utilized to assess cognitive workload during a monitoring task, such as air traffic controller surveying airplane flight processes, to support or warn operators for cognitive exhaustion. Alternatively, workload can be dispatched to a colleague who does not have to cope with high workload during work. Since objects of interest can be visualized using a small moving circle, smooth pursuit eye movements can be triggered this way. As a result, accidents, which occur due to mental overload, distractions, or fatigue, can be avoided. For example, the user interface can be adapted by simplifying displayed content or dispatching a part of the observation task to another colleague. This use case is transferable to other applications, where moving objects occur naturally and require permanent attention of the user. Figure~\ref{fig:teaser_air_tower} shows an example of how smooth pursuit can be used in such situations.

\subsection{Adaptation of Pursuit-based Interactive Systems}
Prior research has introduced many applications that use smooth pursuit primarily for interaction. As we illustrated in our related work section, smooth pursuit interfaces have been used for smartwatch interaction \cite{esteves2015orbits} and interaction with smartphones~\cite{Liu2015}. Using mobile devices enables ubiquitous sensing of cognitive workload in outdoor settings, bypassing the disadvantages of using pupillary measures being prone to lighting conditions. Interacting with large distant displays \cite{vidal2013pursuits}, where touch and gesture interaction have emerged as state of the art to communicate input~\cite{Peltonen:2008:MDT:1357054.1357255, Vogel:2004:IPA:1029632.1029656} can use smooth pursuit to implicitly measure mental states.

Our approach enables implicit contactless assessment of cognitive workload while interacting with these devices. Pursuit-based interactive systems benefit from our classifier to dynamically predict the current cognitive workload level of the user during interaction and adapt to it accordingly. If high task load is identified during an interaction, the user interface or task objective can be modified by an easier one. Figure~\ref{fig:teaser_public_display} shows how the existence of cognitive workload can be estimated to adapt a public display app.

\begin{figure}
    \centering
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/teaser_flight_control_tower4.png}
        \label{fig:teaser_public_display}}
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/teaser_public_display5.png}
        \label{fig:teaser_air_tower}}
    \caption[Exemplary use cases for smooth pursuit-based workload assessments]{\textbf{(a):} User working in an air control tower. Moving dots representing airplanes on the screen can cause smooth pursuit eye movements. (A) The system detects high cognitive workload from the user and dispatches some observation tasks to a colleague. (B) Alleviated cognitive workload measured after user interface adaption. \textbf{(b):} User playing a quiz game on a public display. The system infers that the question is inducing high cognitive workload. The system is, therefore, observing if this behavior persists and provides a hint to avoid frustration.}
    \label{fig:teaser_sp}
\end{figure}


\section{Study Conclusion}
The presented study investigated the influence of cognitive workload on smooth pursuit eye movements using three different trajectories with two different velocities. Using an auditory delayed digit recall \textit{N}-back task to induce cognitive workload, a higher deviation of gaze points from shown trajectories is measured compared to measurements when not inducing cognitive workload. Based on our results, we create a person-independent classifier for estimating binary workload and a person-dependent classifier for distinguishing different levels of cognitive workload. While binary cognitive workload classification can be elicited in the public using smooth pursuit interfaces, private spaces benefit from person-dependent classifier calibration to determine different levels of cognitive workload. The collected data set is available on Github\footnote{\url{www.github.com/hcum/your-eyes-tell} - last access \urldate}.

% Having such a measurement modality without the need of body-worn devices goes a step towards real-time mental state estimation in ubiquitous computing environments. User interfaces can then provide intervention mechanisms to relax or help users based on their current context. Our classifier depends on eye gaze only and fits into several application scenarios. It can be deployed in real-world scenarios to estimate the presence of cognitive workload in real-time. Thereby, the assessment can be done contactless without the need for additional bodyworn sensors.

% In future work, we plan to focus on specific use cases which leverage smooth pursuit as interaction modality to provide an assessment of cognitive workload in real-time. This input will be used to adapt to user interfaces of applications accordingly. This includes implementations on public and head-mounted displays using smooth pursuit as input. Furthermore, we want to evaluate the efficiency of assessing cognitive workload unconsciously in user interfaces which naturally display moving elements. This comprises monitoring tasks, which can be found in air traffic and train control systems. Consequently, such systems can be benchmarked and optimized regarding their usage complexity. To complement this, further research aiming to correlate objective and subjective workload measures, such as eye movement deviations and NASA-TLX questionnaires, will be conducted. Finally, we will investigate how multiple displayed moving stimuli will affect the classification performance and subjective perception of cognitive workload.
% To encourage research in this area, we published the data set for further analysis by the research community on our institute's homepage\footnote{\url{www.hcilab.org/your_eyes_tell_data_set} - last access 2018-01-08}.

\section{Chapter Conclusion}
In this chapter, we investigated the characteristics of eye movements during different levels of cognitive workload. Eye movements can be recorded using a remote eye tracker which obviates direct body contact with the user. We show that cognitive workload levels can be classified using specific smooth pursuit eye movements using machine learning techniques. Contrary to \ac{EEG}, no calibration procedure or tedious setup is required. Thus, the real-time analysis of eye movement holds promise as an additional measurement channel for workload-aware computing interfaces.

Having such a measurement modality without the need of body-worn devices goes a step towards real-time mental state estimation in ubiquitous computing environments. User interfaces can then provide intervention mechanisms to relax or help users based on their current context. Our classifier depends on eye gaze only and fits into several application scenarios. It can be deployed in real-world scenarios to estimate the presence of cognitive workload in real-time. Thereby, the assessment can be done without the need for contact or additional bodyworn sensors, which comes closer to Mark Weiser's vision of ubiquitous computing. However, the classification performance varied throughout the displayed trajectories, and for both person-dependent and person-independent cases. Whereas accuracies of up to 99\% can be achieved for binary person-independent classification, person-dependent classification excels at the classification for different \textit{N}-back difficulties. Workload-aware interfaces that are deployed in the public may benefit from cognitive workload estimation using a binary classification whereas it may be acceptable to calibrate for fine-grained workload determination in private spaces. This chapter answers \textbf{RQ4} with the focus of measurable changes in smooth pursuit eye movements, which can be leveraged by workload-aware systems for cognitive workload classification.

\chapter{Pupil Dilation}
\label{ch:pupil_dilation}

%\epigraph{\textit{The soul, fortunately,\\ has an interpreter, \\ often an unconscious, \\but still a faithful interpreter, \\in the eye.}}{Charlotte Brontë, Jane Eyre}
\setlength{\epigraphwidth}{6.5cm}
\epigraph{\textit{Sitting in the far horizon\\
The evergreens across the border\\
Can you see a different story\\
With the failure and the glory\\
The truth is in the eyes of the beholder\\
The truth is in her eyes when you hold her
}}
{Andrew Stockdale}

The previous chapter investigated changes in eye movements during different levels of cognitive workload. An \textit{N}-back task was employed to elicit different levels of cognitive workload. Specifically smooth pursuit eye movements were affected and could be successfully classified between and within persons. However, moving elements are required to elicit smooth pursuit movements since they cannot be pretended or simulated by humans~\cite{velloso2016ambigaze}. Alternative metrics for measuring cognitive workload using eye-based properties have found relevance in previous research~\cite{duchowski2002breadth, duchowski2018gaze} including pupil dilation.

% Context-aware computing has grown in recent years, proliferating devices and day-to-day life. Adapting system behavior according to location, physical activity, or social interactions is accepted and often expected by users. Sensing emotional states has attracted attention as a modality for context-aware computing and has been researched thoroughly in the domain of affective computing~\cite{bulling2014tutorial, tao2005affective}. Additionally, the analysis of cognitive processes has great potential for providing adapted content from a mental point of view \cite{bulling2014cognition}. Such cognition-aware systems analyze cognitive processes, derive implications from psycho-physiological states, and provide tailored content based on the user's cognitive state. Various experiments in Human-Computer Interaction (HCI) depend on measures for quantifying cognitive effort. To specify the complexity of experimental conditions, questionnaires such as the NASA-TLX \cite{hart2006nasa, hart1988development} or the Driver Activity Load Index \cite{pauzie2008method}, are used to derive cognitive implications which depend on subjective perceptions of participants. However, these measures of mental task complexities are often generalized for all participants, leading to a lack of individual user-dependent cognition-awareness for later designed systems.

% \begin{figure}
%  \centering
%  \includegraphics[width=1.0\marginparwidth]{figures/chapter_eye_tracking/pupil_compared}
%  \caption{Exemplary impact of cognitive workload on pupil dilation. \textbf{Top:} Measured pupil diameter under low cognitive workload. \textbf{Bottom:} Measured pupil diameter under high cognitive workload.}
%  \label{fig:pupil_compared}
% \end{figure}

\begin{figure}[h!]
    \centering
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/pupil_low_edited.png}
        \label{fig:pupil_low}}
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/pupil_high_edited.png}
        \label{fig:pupil_high}}
    \caption[Pupil dilation under different levels of workload]{Exemplary impact of cognitive workload on pupil dilation. \textbf{(a):} Measured pupil diameter under low cognitive workload. \textbf{(b):} Measured pupil diameter under high cognitive workload.}
    \label{fig:pupil_compared}
\end{figure}

Pupil dilation has attracted attention in the HCI community as a measure for cognitive workload (see Figure \ref{fig:pupil_compared})~\cite{Duchowski:2018:IPA:3173574.3173856}. Demanding the short-term memory frequently over a timespan causes cognitive effort~\cite{ashcraft2001relationships, ashcraft2007working, heitz2008effects, hess1964pupil, kahneman1966pupil}, a mental process which extends the pupil diameter (see Figure~\ref{fig:pupil_high}). Eye trackers are used to retrieve eye gaze positions which can be used at the same time to evaluate pupillary data in real-time. Using such a metric as an assessment of cognitive workload can be utilized by applications to provide help and assistance for users when high cognitive workload is detected. For example, workload-aware systems can assist in real-time during a cognitively demanding task. Furthermore, the usability of interfaces can be evaluated by conjunctively assessing pupil diameter and eye gaze during user interaction. Although being sensitive to lighting conditions, the evaluation of pupil dilation to infer cognitive workload has been examined by various researchers. Benedetto et al.~\cite{benedetto2011driver} explored the impact of cognitive workload on pupil dilation and eye blink duration. Since pupillary measurements are error-prone to lighting conditions, Pfleging et al. \cite{pfleging2016model} proposed a model for classifying cognitive workload of pupil dilation under different lighting conditions. Kiefer et al.~\cite{kiefer2016measuring} evaluated the pupil diameter under different task difficulties to assess the perceived task complexity. Gollan et al.~\cite{Gollan:2016:DEC:2968219.2968550} examined the assessment of pupil dilation under cognitive workload in real-time. Hess et al. \cite{hess1964pupil} investigated the impact of simple mental processes, such as solving one and two-digit multiplications, on the pupil diameter. Zbrodoff and Logan \cite{zbrodoff2005everyone} found a correlation between higher pupil extensions and increasing math exercise complexity. By using multiplication tasks, a higher pupil diameter was measured when multiplying two-digit numbers than one-digit numbers.

This chapter investigates the performance of a classification model that distinguishes between two different levels of workload. This includes the assessment of pupil dilation to create adaptive workload-aware interfaces that adjust the difficulty in real-time. Thereby, task complexity is set to a suitable difficulty to keep users engaged, thus becoming more difficult or easier depending on current mental workload measurements. This is complemented by presenting and evaluating a proof-of-concept application, which sets its task complexity based on pupillary data to prevent mental underload or overload. Hence, this chapter complements the second part of the research question:

%Previous work has explored the influence of changing pupil diameters during different task complexities and possibilities to classify cognitive workload based on pupil extensions. However, the presented theoretical concepts have not been evaluated in the context of a real-world task, where the complexity of the presented content is adapted according to the mental resources of the user. In our work, we investigate the impact of adjusting the complexity of a cognitive inducing task in real-time using pupillary data. Task complexity is set to a suitable difficulty to keep users engaged, thus becoming more difficult or easier depending on current mental workload measurements. This is complemented by presenting and evaluating a proof-of-concept application, which sets its task complexity based on pupillary data to prevent mental underload or overload.

\begin{itemize}%[leftmargin=1em]
    \renewcommand{\labelitemi}{$\rightarrow$}
   \item \textbf{RQ4}: Do eye gaze metrics enable the classification of cognitive workload states?
\end{itemize}

\begin{center}
    \begin{GrayBox}
        \centering
        \parbox{0.98\textwidth}{
            \emph{This section is based on the following publication:}
            \vspace{3mm}
            \publicationsbegin    
            \item \bibentry{Kosch:2018:LME:3170427.3188643}
            \publicationsend
        }
    \end{GrayBox}
\end{center}

\section{Application}
To examine the usefulness of adapting task complexity based on pupillary data, we constructed a prototype capable of evaluating pupil dilation measurements in real-time.

\subsection{Recording and Feedback Setup}
A mobile eye tracker from Pupil Labs\footnote{\url{www.pupil-labs.com} - last access \urldate} is used to receive pupillary data. Data was updated at 30\,Hertz and processed on the attached computer. An external screen is used to display stimuli. To avoid distractions during the experiment, the setup was divided into two areas using separators, respectively for the experimenter and participant. The experiment was conducted in a room without windows and constant lighting conditions. The stimulus monitor had a resolution of $1920\times1080$ and a screen size of $23$ inches.
%\begin{figure}
%  \includegraphics[width=1.0\columnwidth]{figures/experiment_construction}
%  \caption{Pilot study setup using separators. \textbf{Left:} Participant side provided with a monitor and keyboard. \textbf{Right:} Experimenter side equipped with a computer to monitor the study.}
%  \label{fig:experiment_construction}
%\end{figure}

%\begin{figure}
%  \includegraphics[width=1.0\columnwidth]{figures/mathtask}
%  \caption{Multiplication math task with equations moving from top to bottom comprising two different difficulties. \textbf{Left:} Simple multiplication containing one-digit numbers. \textbf{Right:} Difficult multiplication comprising a two-digit number and a one-digit number.}
%  \label{fig:mathtask}
%\end{figure}

%\marginpar{%
%\justify
%  \vspace{-18em}
% \fbox{%
%  \begin{minipage}{0.925\marginparwidth}
%We trained a person-dependent \textbf{SVM classifier} with a linear kernel to infer required changes of task difficulty in real-time. We used the individual pupil dilation as the only feature. We defined two classes, easy and difficult. The classifier was trained individually for every participant after the two baseline trials. In the last trial, the previously trained classifier is used to predict cognitive workload. The task difficulty is set to the opposite task complexity to force cognitive alleviation or effort. The person-dependent classifier accuracies ranged between 64$\%$ and 99$\%$ ($M = 79\%$, $SD = 0.16\%$) resulting from a k-fold cross-validation with $k=5$.
%
%\end{minipage}}
%\label{sec:features} }

\subsection{Classifier}
Two baseline trials are conducted in the beginning to obtain ground truth data about pupil dilation during an \textit{easy} and a \textit{difficult} math task, each lasting three minutes. A single complexity was assigned to every trial (\textit{easy}/\textit{difficult}). The trained classifier is then used to adaptively control the complexity of the displayed multiplications in a third trial. The classifier aims to estimate low and high cognitive workload based on the data retrieved from the two baseline tasks. The prototype simulates a cognition-aware system by setting task complexity to \textit{easy} if high mental workload is measured. In contrast, task complexity is set to \textit{difficult} when low cognitive workload is classified from the previous baseline measurements. 

To assess cognitive workload from the users' pupil dilation, we trained individual support vector machines (SVMs) with a linear kernel to infer required changes of task difficulty in real-time. We used the individual pupil dilation as the only feature. We defined two classes, \textit{easy} and \textit{difficult}. The classifier was trained individually for every participant after the two baseline trials. In the last trial, the previously trained classifier is used to predict cognitive workload. The task difficulty is set to the opposite task complexity to force cognitive alleviation or effort. The person-dependent classifier accuracies ranged between 64$\%$ and 99$\%$ (M = $79\%$, SD = $0.16\%$) resulting from a k-fold cross-validation with $k=5$.

\section{Study}
We conducted a pilot study to evaluate the feasibility of changing task complexity based on pupil diameter measurements as an indicator for cognitive workload. The study configuration conforms to the previously described prototype.

\subsection{Cognitive Task}
To induce cognitive workload, we use a multiplication math task with two different complexity levels including one-digit and two-digit multiplications. Both complexities lead to different pupil dilations~\cite{ashcraft2001relationships, ashcraft2007working, zbrodoff2005everyone}. To add a time constraint, the multiplication math tasks were moving centered from the top to the bottom of the screen within five seconds. During the time limit, participants were asked to type the correct solution on a keyboard number pad. When the multiplication reached the bottom of the screen, it disappeared and a new multiplication is displayed at the top of the screen. If the user fails to enter a solution during the given time frame, an error is counted. If the solution entered during the time is correct, the multiplication disappears and a new multiplication task is displayed at the top of the screen. The complexity is divided into \textit{easy} and \textit{difficult}. The \textit{easy} condition uses numbers ranging from $0 - 9$, randomly selecting two numbers which have to be multiplied together. In the \textit{difficult} condition, two numbers are randomly chosen, where the first number ranges from $10 - 19$ and the second from $0 - 9$ (see Figure \ref{fig:mathtask}). Numbers are constantly displayed in black font on a gray background (RGB: $[150, 150, 150]$).

\subsection{Participants}
Six participants (4 male, 2 female) took part in the pilot study, ranging from an age between 22 and 34 years (M = $29.17$, SD = $4.41$). All participants were computer science, students or researchers. Participants had a normal or corrected-to-normal vision. The overall duration of the study was approximately 15 minutes. Before the start of the experiment, participants signed an informed consent form and provided their demographic data.

\begin{figure}
    \centering
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/mathtask_easy.png}
        \label{fig:math_easy}}
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/mathtask_difficult.png}
        \label{fig:math_high}}
    \caption[Math task employed during the experiment]{Multiplication math task with equations moving from top to bottom comprising two different complexities. \textbf{(a):} \textit{Easy} multiplication containing one-digit numbers. \textbf{(b):} \textit{Difficult} multiplication comprising a two-digit number and a one-digit number.}
    \label{fig:mathtask}
\end{figure}

\subsection{Procedure}
First, we explained to the participants the study procedure and familiarized them with the setting. The mobile eye tracker was then calibrated. The study consisted of three trials; two baseline multiplication trials (\textit{easy}/\textit{difficult}) and one \textit{adaptive} multiplication trial. The duration of each task was three minutes. The order of the first two baseline trials was counterbalanced according to the balanced Latin square. The pupillary data from the baseline tasks was used to derive an SVM classifier capable to distinguish between cognitive workload induced by a \textit{easy} or \textit{difficult} task. During the \textit{adaptive} trial, the trained user-dependent classifier is used to adaptively set the complexity of the multiplication task. The complexity is set by classifying measured pupil diameter data in five-second intervals. If the classifier estimates a high diameter difference, the task complexity is set to \textit{easy} to avoid mental overload. In contrast, the task complexity is set to \textit{difficult} if the classifier estimates a low pupil diameter to avoid mental underload. If the classifier determines a complexity change during a multiplication task, the new task complexity is adjusted to the next appearing multiplication. After every trial, participants filled a NASA-TLX \cite{HART1988139} questionnaire to obtain subjectively perceived workload during the trials.

\section{Exploratory Results}
Overall, the \textit{easy} multiplication condition consisted of $618$ displayed calculations, the \textit{difficult} condition $420$ displayed multiplications, and $466$ displayed calculations for the \textit{adaptive} condition. Least errors were measured during \textit{easy} multiplication, comprising $571$ correct ($92$\%) and $47$ wrong ($8$\%) answers. Most errors were made during \textit{difficult} trials with $255$ correct ($61$\%) and $165$ wrong ($39$\%) answers. The \textit{adaptive} condition placed itself in between with $313$ correct ($67$\%) and $153$ wrong ($33$\%) answers.

% \begin{figure}
% \justify
%  \includegraphics[width=1.0\columnwidth]{figures/chapter_eye_tracking/averaged_pupil_plot3.pdf}
% \vspace*{-9.5mm}
% \caption{Averaged differences of pupil diameter per participant between \textit{easy} and \textit{difficult} task complexities as well as \textit{easy} and \textit{adaptive} task complexities. The difference between the \textit{easy} and \textit{difficult} task complexity is higher compared to the \textit{adaptive} task complexity except for two participants (p5, p6). The whisker lines depict the standard error.}
%  \label{fig:averaged_pupil_plot}
%  \vspace{-1em}
% \end{figure}

\begin{figure}
    \centering
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/averaged_pupil_plot3.pdf}
        \label{fig:averaged_pupil_plot}}
    \subfloat[][]{
        \includegraphics[width=0.5\columnwidth]{figures/nasa_tlx_score3.pdf}
        \label{fig:nasa_tlx_score}}
    \caption[Pupil diameter differences and raw NASA-TLX scores]{\textbf{(a):} Averaged differences of pupil diameter per participant between \textit{easy} and \textit{difficult} task complexities as well as \textit{easy} and \textit{adaptive} task complexities. The difference between the \textit{easy} and \textit{difficult} task complexity is higher compared to the \textit{adaptive} task complexity except for two participants (p5, p6). The whisker lines depict the standard error. \textbf{(b):} Averaged NASA-TLX scores for the different task difficulties. The whisker lines depict the standard error.}
    \label{fig:results_pupil}
\end{figure}

We investigate individual differences in the pupil dilation measures between the different task complexities. The differences in the \textit{easy} and \textit{difficult} task complexity ranged between $0.05$ and $0.87$ millimeters. The difference between the \textit{easy} and \textit{adaptive} complexity ranged between $0.05$ and $0.85$ millimeters. Figure \ref{fig:averaged_pupil_plot} shows the difference between the averaged pupillary measurements per participant. The mean number of complexity switches during the \textit{adaptive} condition results in $2.6$ complexity changes for a total of $466$ multiplication tasks during the \textit{adaptive} condition. The mean NASA-TLX score (see Figure~\ref{fig:nasa_tlx_score}) reveals lowest subjectively perceived workload during the \textit{easy} condition (M = $9.75$, SD = $1.45$) and highest workload measurements during the \textit{difficult} complexity (M = $12.05$, SD = $2.15$). The \textit{adaptive} condition was rated between both baseline trials (M = $11.30$, SD = $2.14$).

\section{Discussion}
In this study, we explored the impact of adapting the complexity of a cognitive workload inducing task based on the measurement of pupillary changes.

\subsection{Adaptive User Interfaces}
Our findings support the use of pupil dilation to detect mental effort. Assessing mental workload in real-time to change the task complexity has shown its feasibility when participants performed adapted math tasks. The adaptive trial shows how computing systems can make use of the pupil diameter to create engaging user interfaces while avoiding the perception of high or low mental workload.
\subsection{Creating User Specific Models}
The study shows the viability of individually trained classifiers. Since physiological measurements differ among users, person-dependent measurements cannot be avoided. Limited to pupillary data, encouraging results were achieved by allocating short training times to create a user-specific model. This is supported by averaged pupil diameter measurements and subjective feedback provided through NASA-TLX questionnaires.

% \begin{figure}
% \justify
%  \includegraphics[width=\columnwidth]{figures/chapter_eye_tracking/nasa_tlx_score3.pdf}
%  \vspace*{-9mm}
%  \caption{Averaged NASA-TLX scores for the different task difficulties. The whisker lines depict the standard error.}
%  \label{fig:nasa_tlx_score}
%  \vspace{-5mm}
% \end{figure}

\section{Study and Chapter Conclusion}
This chapter investigated the assessment of cognitive workload based on pupillary data to change the complexity of a task in real-time. In a preliminary study, we trained person-dependent classifiers through math tasks with different complexities. During an \textit{adaptive} trial, task complexity was changed depending on the classification of pupillary data. The results show the practicability of using pupillary data in controlled environments to evaluate user interface adaptation mechanics and user interface assessment. 

Eye gaze-based properties reflect cognitive states. In this chapter, we investigated the suitability of pupil dilation as an alternative workload measure. A simple classification scheme revealed reliable discrimination between low and high workload states for difficulty alternations, hence assessing pupil dilation as a suitable measure for cognitive workload (\textbf{RQ4}). Performance and subjective reports imply that more engagement and less frustration is fostered when alternating between task difficulties. In contrast to smooth pursuit, dilation-based workload assessments do not require a moving object to be detected. However, while not being affected by moving objects, the pupil size is sensitive to light conditions. The presented experiment leveraged a controlled setup to avoid bias through lighting conditions. A potential solution is the normalization of pupil dilation through in-situ light measurements. The combination of lighting conditions and pupil dilation can provide a decent estimate for the currently perceived workload.


==> chapter/relatedwork.tex <==
% !TEX root = ../thesis.tex

%there are no parts 
%\part{Introduction and Background\label{part-1-introduction}}


\chapter{Related Work}
\todo{20 pages}

\section{Cognitive Augmentation}

\subsection{Feedback Mechanisms}

\todo{Include AI}

\subsection{Multimodal Assistive Computing}

\section{Domain-Specific Cognitive Assistance}

\subsection{Assistance in Industrial Environments}

\subsection{Assistance for Cognitively Impaired}

\section{Physiological Sensing for Assistive Technologies}

\subsection{Advances in Artificial Intelligence}
\todo{part on AI}

\subsection{System Adaptation}
\todo{closed feedback loop}

\section{Contribution}
\todo{summarize gap between previous and current research}

==> tex/00_coauthorship.tex <==
\newcommand{\forceindent}{\leavevmode{\parindent=3em\indent}}

\specialchapter{Publications and Declaration of Co-Authorship}

All the following papers were peer-reviewed. 

\textbf{Chapter~\ref{chap:pdapps}}

Chapter~\ref{chap:pdapps} corresponds to the following workshop paper:

\begin{adjustwidth}{2cm}{}
Mohamed Khamis, Andreas Bulling, Florian Alt. \textbf{Tackling Challenges of Interactive Public Displays using Gaze.} In Adj. Proc.\,of the ACM International Joint Conference on Pervasive and Ubiquitous Computing (UbiComp 2015), pp. 763-766, 2015.
\end{adjustwidth}


i did this they did that... 

\textbf{Chapter~\ref{chap:eyepact}}

Chapter~\ref{chap:eyepact} corresponds to the following journal paper:




\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Daniel Buschek, Tobias Thieron, Florian Alt, Andreas Bulling. \textbf{EyePACT: Eye-Based Parallax Correction on Touch-Enabled Interactive Displays.} In Proc.\,ACM Interact.\,Mob.\,Wearable Ubiquitous Technol.\,(IMWUT) 1, 4, December 2017, 18 pages.
\end{adjustwidth}


i did this they did that... 


\textbf{Chapter~\ref{chap:gtmopass}}

Chapter~\ref{chap:gtmopass} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Regina Hasholzner, Andreas Bulling, Florian Alt. \textbf{GTmoPass: Two-factor Authentication on Public Displays Using GazeTouch passwords and Personal Mobile Devices.} In Proceedings of the 6th International Symposium on Pervasive Displays (PerDis 2017).
\end{adjustwidth}


i did this they did that... 




\textbf{Chapter~\ref{chap:eyescout}}

Chapter~\ref{chap:eyescout} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Axel Hoesl, Alexander Klimczak, Martin Reiss, Florian Alt, Andreas Bulling. \textbf{EyeScout: Active Eye Tracking for Position and Movement Independent Gaze Interaction with Large Public Displays.} In Proceedings of the 30th Annual ACM Symposium on User Interface Software \& Technology (UIST 2017).
\end{adjustwidth}


i did this they did that... 


\textbf{Chapter~\ref{chap:calibration}}

Section~\ref{sec:textpursuits} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Ozan Saltuk, Alina Hang, Katharina Stolz, Andreas Bulling, Florian Alt. \textbf{TextPursuits: Using Text for Pursuits-Based Interaction and Calibration on Public Displays.} In Proc.\,of the 2016 ACM International Joint Conference on Pervasive and Ubiquitous Computing (UbiComp 2016).
\end{adjustwidth}


i did this they did that... 


Section~\ref{sec:eyevote} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Ludwig Trotter, Markus Tessmann, Christina Dannhart, Andreas Bulling, Florian Alt. \textbf{EyeVote in the Wild: Do Users bother Correcting System Errors on Public Displays?} In Proc.\,of the 15th International Conference on Mobile and Ubiquitous Multimedia (MUM 2016).
\end{adjustwidth}


i did this they did that... 


% \textbf{Chapter~\ref{chap:multipleusers}}

% Chapter~\ref{chap:multipleusers} corresponds to the following conference paper:

% \begin{adjustwidth}{2cm}{}
%     TBA
% \end{adjustwidth}


\vspace{2cm}
Munich, 15.12.2017 
\hfill{\rule{4cm}{1pt}}

\hfill{Mohamed Khamis}
